Transfer Learning with Convolutional Networks for Atmospheric Parameter Retrieval

The Infrared Atmospheric Sounding Interferometer (IASI) on board the MetOp satellite series provides important measurements for Numerical Weather Prediction (NWP). Retrieving accurate atmospheric parameters from the raw data provided by IASI is a large challenge, but necessary in order to use the data in NWP models. Statistical models performance is compromised because of the extremely high spectral dimensionality and the high number of variables to be predicted simultaneously across the atmospheric column. All this poses a challenge for selecting and studying optimal models and processing schemes. Earlier work has shown non-linear models such as kernel methods and neural networks perform well on this task, but both schemes are computationally heavy on large quantities of data. Kernel methods do not scale well with the number of training data, and neural networks require setting critical hyperparameters. In this work we follow an alternative pathway: we study transfer learning in convolutional neural nets (CNN s) to alleviate the retraining cost by departing from proxy solutions (either features or networks) obtained from previously trained models for related variables. We show how features extracted from the IASI data by a CNN trained to predict a physical variable can be used as inputs to another statistical method designed to predict a different physical variable at low altitude. In addition, the learned parameters can be transferred to another CNN model and obtain results equivalent to those obtained when using a CNN trained from scratch requiring only fine tuning.

==> Conv_table_summary.tex <==
\begin{table*}[h!]
\centering
\caption{Table of CNN architectures developed in this work. Training times are reported on a Python (Theano) implementation running on a single NVIDIA Titan Black GPU.}% Convnet C is reported with mean and standard deviation over training with 5 random initializations.} %A full architecture description is found in the Appendi$\times$. GUS: it's not common to include such short appendi$\times$ in these RS journals...
\label{tb:conv_summ}
\begin{tabular}{|l|l|l|l|l|}
\hline
 & CNN A & CNN B & CNN C & CNN D\\
\hline
\hline
Input Size & 125$\times$3$\times$3 & 125$\times$10$\times$10 & 125$\times$15$\times$15 & 125$\times$25$\times$25\\
Number of layers & 4 & 6 & 6 & 7 \\
Number of parameters & 127,290 & 347,070 & 639,750 & 938,350 \\
\hline
Output dimension & \multicolumn{4}{|c|}{90} \\
\hline
Optimizer & \multicolumn{4}{|c|}{ADAM \cite{kingma2014adam}} \\
\hline
Approx. Training time & 4h & 11h & 18h & 39h \\
\# train. samples & 524,552 & 460,887 & 415,472 & 324,792 \\
\hline
Mean test RMSE [K] & 2.48 & 2.43 & 2.19 & 2.28 \\
\hline
\end{tabular}
\end{table*}



==> Convnet_table.tex <==
\begin{table*}[h!]
\centering
\caption{Table of CNN architectures. B.R.D. is a concatenation of 3 layers, Batch Normalization, Rectified Linear Unit activation layer and Dropout. Dropout is performed with a probability $p=0.5$ in all cases. The parameter column denote (number of channels in previous layer) x (filters in this layer) x (filter height) x (filter width).}
\label{tb:fullconvnet}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\multicolumn{3}{|c|}{CNN A} & \multicolumn{3}{c|}{CNN B} \\
\hline
\hline
Type & Parameters & Output & Type & Parameters & Output \\
\hline
Input & - & 125x3x3 &           Input & - & 125x10x10  \\
Conv & 125x60x3x3 & 60x1x1 &    Conv & 125x60x3x3 & 60x10x10 \\
B.R.D. & - & 60x1x1 &           Conv & 60x60x3x3 & 60x10x10 \\
Conv &  60x120x1x1 & 120x1x1 &  Pool & - & 60x5x5 \\
B.R.D. & - & 120x1x1 &          B.R.D. & - & 60x5x5  \\
Conv & 120x240x1x1 & 240x1x1 &  Conv & 60x120x3x3 & 120x5x5 \\
B.R.D. & - & 240x1x1 &          Conv & 120x120x3x3 & 120x3x3  \\
Conv & 240x90x1x1 & 90x1x1 &    Pool & - & 120x1x1  \\
 &  &  &                        B.R.D. & - & 120x1x1  \\
 &  &  &                        Conv & 120x240x1x1 & 240x1x1 \\
 &  &  &                        B.R.D. & - & 240x1x1  \\
 &  &  &                        Conv & 240x90x1x1 & 90x1x1  \\
\hline
\end{tabular}
\vskip 10pt
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\multicolumn{3}{|c|}{CNN C} & \multicolumn{3}{c|}{CNN D}\\
\hline
\hline
Type & Parameters & Output & Type & Parameters & Output \\
\hline
Input & - & 125x15x15 &             Input & - & 125x25x25 \\
Conv & 125x100x3x3 & 100x15x15 &    Conv & 125x100x3x3 & 100x23x23 \\
Conv & 100x100x3x3 & 100x13x13 &    Conv & 100x100x3x3 & 100x21x21 \\
Pool & - & 100x6x6 &                Pool & - & 100x10x10 \\
B.R.D. & - & 100x6x6 &              B.R.D. & - & 100x10x10 \\
Conv & 100x160x3x3 & 160x4x4 &      Conv & 100x160x3x3 & 160x8x8 \\
Conv & 160x160x3x3 & 160x2x2 &      Conv & 160x160x3x3 & 160x6x6 \\
Pool & - & 160x1x1 &                Pool & - & 160x3x3 \\
B.R.D. & - & 160x1x1 &              B.R.D. & - & 160x3x3 \\
Conv & 160x240x1x1 & 240x1x1 &      Conv & 160x200x3x3 & 200x1x1 \\
B.R.D. & - & 240x1x1 &              B.R.D. & - & 200x1x1 \\
Conv & 240x90x1x1 & 90x1x1 &        Conv & 200x240x1x1 & 240x1x1 \\
 &  &  &                            B.R.D. & - & 240x1x1 \\
 &  &  &                            Conv & 240x90x1x1 & 90x1x1 \\
\hline
\end{tabular}
\end{table*}

